Volt/VAR Optimization in Transmission Networks with Discrete-Control Devices

Voltage (Volt) and reactive-power (VAR) control in transmission networks is critical for reliability and increasingly needs fast, implementable decisions. This paper presents a transmission Volt/VAR Optimization (VVO) framework that co-optimizes discrete control of on-load tap-changing transformers (OLTCs) and capacitor banks (CBs) with AC power flow (ACPF) physics to improve voltage stability and minimize VAR generation. The framework follows a relax-round-resolve pipeline: a continuous relaxation proposes targets, a rounding step selects feasible discrete settings, and a final solve enforces AC power flow physics. Extensive experiments on IEEE, PEGASE, and RTE systems show consistent improvements in voltage and VAR quality metrics with modest generator redispatch while preserving economic operation and achieving compatible runtimes with real-time transmission operations.

==> tex/definitions.tex <==
\RequirePackage{amsmath,amssymb}
\RequirePackage{bm}

% --- Style helpers ---
\newcommand{\bv}[1]{\mathbf{#1}}   % bold roman
\newcommand{\vect}[1]{\bm{#1}}     % bold greek
\newcommand{\lb}[1]{\underline{#1}}
\newcommand{\ub}[1]{\overline{#1}}
\newcommand{\set}[1]{\mathcal{#1}}
\newcommand{\acopf}[1]{\hat{#1}}       % ACOPF solution
\newcommand{\rvvo}[1]{\overline{#1}}   % Relaxed VVO solution

\newcommand{\im}{\mathbf{j}}  % imaginary unit

% --- Sets ---
\newcommand{\NODES}{\set{N}}
\newcommand{\EDGES}{\set{E}}
\newcommand{\LOADS}{\set{L}}
\newcommand{\GENERATORS}{\set{G}}

% --- Device-location subsets ---
\newcommand{\TAPEDGES}{\mathcal{T}} % branches with on-load tap changers (OLTC), indices ij
\newcommand{\CBNODES}{\mathcal{B}}   % buses equipped with capacitor banks, indices i
% Per-bus
\newcommand{\Gi}{\GENERATORS_i}
\newcommand{\Li}{\LOADS_i}
\newcommand{\Eiplus}{\EDGES_i^{+}}
\newcommand{\Eiminus}{\EDGES_i^{-}}

% --- Variables ---
\newcommand{\V}{\bv{V}} % voltage phasor including magnitude and angle
\newcommand{\VM}{\bv{v}}
\newcommand{\VA}{\vect{\theta}}
\newcommand{\DVA}{\Delta\vect{\theta}} % branch angle difference
\newcommand{\SG}{\bv{S}^{\text{g}}} % generator apparent power
\newcommand{\PG}{\bv{p}^{\text{g}}}
\newcommand{\QG}{\bv{q}^{\text{g}}}
\newcommand{\PF}{\bv{p}^{\text{f}}}
\newcommand{\QF}{\bv{q}^{\text{f}}}
\newcommand{\PT}{\bv{p}^{\text{t}}}
\newcommand{\QT}{\bv{q}^{\text{t}}}
\newcommand{\CB}{\boldsymbol{\beta}} % number of active capacitor bank modules
\newcommand{\TAP}{\boldsymbol{\tau}} % tap ratio defined as nominal + tap_position*tap_step
\newcommand{\Ybr}{\bv{Y}^{\mathrm{br}}} % branch admittance matrix
\newcommand{\PFSOL}{\bv{x}}

% --- Apparent Power variables ---
\newcommand{\SF}{\bv{S}^{\mathrm{f}}} % apparent power flow - from
\newcommand{\ST}{\bv{S}^{\mathrm{t}}} % apparent power flow - to

% --- Parameters ---
% --- Line ---
\newcommand{\gij}{g_{ij}} % line susceptance
\newcommand{\bij}{b_{ij}} % line conductance
\newcommand{\yij}{y_{ij}} % line admittance
% To/from admittance values
\newcommand{\yff}{y^{\text{ff}}} % line admittance
\newcommand{\yft}{y^{\text{ft}}} % line admittance
\newcommand{\ytf}{y^{\text{tf}}} % line admittance
\newcommand{\ytt}{y^{\text{tt}}} % line admittance
\newcommand{\gff}{g^{\text{ff}}} % line susceptance
\newcommand{\gft}{g^{\text{ft}}} % line susceptance
\newcommand{\gtf}{g^{\text{tf}}} % line susceptance
\newcommand{\gtt}{g^{\text{tt}}} % line susceptance
\newcommand{\bff}{b^{\text{ff}}} % line conductance
\newcommand{\bft}{b^{\text{ft}}} % line conductance
\newcommand{\btf}{b^{\text{tf}}} % line conductance
\newcommand{\btt}{b^{\text{tt}}} % line conductance
\newcommand{\bcij}{b^{c}_{ij}} % line charging conductance
\newcommand{\st}{\mathrm{st}} % tap step
\newcommand{\smax}{\ub{s}}
\newcommand{\PhaseShift}{\theta^{\mathrm{shift}}}


% --- Bus ---
\newcommand{\gs}{g^{\mathrm{s}}} % shunt conductance
\newcommand{\bs}{b^{\mathrm{s}}} % shunt susceptance
\newcommand{\ys}{y^{\mathrm{s}}} % shunt admittance
\newcommand{\bcb}{b^{\mathrm{cb}}} % capacitor bank per-module susceptance at nominal voltage
\newcommand{\pd}{p^{\mathrm{d}}}
\newcommand{\qd}{q^{\mathrm{d}}}
\newcommand{\Sd}{S^{\mathrm{d}}} % apparent power demand
\newcommand{\cost}{c}

% Reference Values
\newcommand{\vref}{v^{\text{ref}}}
\newcommand{\qgref}{q^{\text{ref}}}
\newcommand{\pgref}{p^{\text{ref}}}
\newcommand{\runtime}{T}

% Solutions of power flow (intermediate steps in the pipeline, not variables)
\newcommand{\pg}{p^{\mathrm{g}}}
\newcommand{\qg}{q^{\mathrm{g}}}
\newcommand{\vm}{v}
\newcommand{\va}{\theta}
\newcommand{\pf}{p^{\mathrm{f}}}
\newcommand{\pt}{p^{\mathrm{t}}}
\newcommand{\qf}{q^{\mathrm{f}}}
\newcommand{\qt}{q^{\mathrm{t}}}

% ACOPF Solution
\newcommand{\pgacopf}{\hat{\bv{p}}^{\mathrm{g}}}
\newcommand{\qgacopf}{\hat{\bv{q}}^{\mathrm{g}}}
\newcommand{\vmacopf}{\hat{\bv{v}}}
\newcommand{\vaacopf}{\hat{\vect{\theta}}}
\newcommand{\pfacopf}{\hat{\bv{p}}^{\mathrm{f}}}
\newcommand{\ptacopf}{\hat{\bv{p}}^{\mathrm{t}}}
\newcommand{\qfacopf}{\hat{\bv{q}}^{\mathrm{f}}}
\newcommand{\qtacopf}{\hat{\bv{q}}^{\mathrm{t}}}
% Relaxed VVO solution
\newcommand{\pgrvvo}{\tilde{\bv{p}}^{\mathrm{g}}}
\newcommand{\qgrvvo}{\tilde{\bv{q}}^{\mathrm{g}}}
\newcommand{\vmrvvo}{\tilde{\bv{v}}}
\newcommand{\varvvo}{\tilde{\vect{\theta}}}
\newcommand{\pfrvvo}{\tilde{\bv{p}}^{\mathrm{f}}}
\newcommand{\ptrvvo}{\tilde{\bv{p}}^{\mathrm{t}}}
\newcommand{\qfrvvo}{\tilde{\bv{q}}^{\mathrm{f}}}
\newcommand{\qtrvvo}{\tilde{\bv{q}}^{\mathrm{t}}}
\newcommand{\TAPrvvo}{\tilde{\TAP}}
\newcommand{\CBrvvo}{\tilde{\CB}}

% --- Bounds ---
\newcommand{\pgmin}{\lb{p}^{\mathrm{g}}}
\newcommand{\pgmax}{\ub{p}^{\mathrm{g}}}
\newcommand{\qgmin}{\lb{q}^{\mathrm{g}}}
\newcommand{\qgmax}{\ub{q}^{\mathrm{g}}}
\newcommand{\vmmin}{\lb{v}}
\newcommand{\vmmax}{\ub{v}}
\newcommand{\dvamin}{\lb{\Delta}\theta}
\newcommand{\dvamax}{\ub{\Delta}\theta}
\newcommand{\tapmin}{\TAP^{\min}}
\newcommand{\tapmax}{\TAP^{\max}}
\newcommand{\cbmin}{\CB^{\min}}
\newcommand{\cbmax}{\CB^{\max}}

% --- Weights ---
\newcommand{\lamv}{\lambda_v}
\newcommand{\lamq}{\lambda_q}
\newcommand{\lamp}{\lambda_p}
\newcommand{\lamc}{\lambda_{c}}

% --- Slack angle ---
\newcommand{\thetaref}{\VA_{\mathrm{ref}}}

